QUILL: Query Intent with Large Language Models using Retrieval Augmentation and Multi-stage Distillation

Large Language Models (LLMs) have shown impressive results on a variety of text understanding tasks. Search queries though pose a unique challenge, given their short-length and lack of nuance or context. Complicated feature engineering efforts do not always lead to downstream improvements as their performance benefits may be offset by increased complexity of knowledge distillation. Thus, in this paper we make the following contributions: (1) We demonstrate that Retrieval Augmentation of queries provides LLMs with valuable additional context enabling improved understanding. While Retrieval Augmentation typically increases latency of LMs (thus hurting distillation efficacy), (2) we provide a practical and effective way of distilling Retrieval Augmentation LLMs. Specifically, we use a novel two-stage distillation approach that allows us to carry over the gains of retrieval augmentation, without suffering the increased compute typically associated with it. (3) We demonstrate the benefits of the proposed approach (QUILL) on a billion-scale, real-world query understanding system resulting in huge gains. Via extensive experiments, including on public benchmarks, we believe this work offers a recipe for practical use of retrieval-augmented query understanding.

==> 5_future_work.tex <==
\section{Future Work}
% This section is not used.

While we have shown big improvements in the end-to-end query classification task, there are many specific areas where we plan to further refine upon.  Starting with the Large Language model, research has shown that a downstream task specific training (sometimes connoted as second stage pretraining) could further help the model.  Even though we have overall gained in performance, we want to close the distillation gap.  There are also use-cases in which offline inference of a very large dataset is needed and in these cases, we need to further improve upon the inference efficiency.  The multi-stage distillation can also be attempted with progressively smaller models (either a mT5-XL to an mT5-large or even mT5-XL to a BERT-based model).  Sampling and curating the data both for enriching the golden data set and for the distillation is also an area for interesting research. Every industry and its use-case have different precision, recall, latency, budget thresholds and this morphs all of the above to an optimization problem.



